Semantic Scaling: Bayesian Ideal Point Estimates with Large Language Models

This paper introduces "Semantic Scaling," a novel method for ideal point estimation from text. I leverage large language models to classify documents based on their expressed stances and extract survey-like data. I then use item response theory to scale subjects from these data. Semantic Scaling significantly improves on existing text-based scaling methods, and allows researchers to explicitly define the ideological dimensions they measure. This represents the first scaling approach that allows such flexibility outside of survey instruments and opens new avenues of inquiry for populations difficult to survey. Additionally, it works with documents of varying length, and produces valid estimates of both mass and elite ideology. I demonstrate that the method can differentiate between policy preferences and in-group/out-group affect. Among the public, Semantic Scaling out-preforms Tweetscores according to human judgement; in Congress, it recaptures the first dimension DW-NOMINATE while allowing for greater flexibility in resolving construct validity challenges.

==> Sections/outline.tex <==


Outline

edits:
- edit model
- include both models?

Intro
    - Text is a particularly promising medium for ideological scaling.
        - Not limited to elite populations (roll call votes or court decisions), but still generated by elites.
        - Is often generated with the purpose of expressing ideology, unlike network based approaches which are more accurately scaling a person's desired social network or information environment.
        - Easily categorized by topic to enable scaling across pre-defined dimensions.
    - However, current methods that use text for scaling struggle to capitalize on this potential.
        - BoW methods like wordfish or wordscores do not directly measure the semantics of a document and attribute any differences in word counts to ideology. Yet, these differences could just as easily be due to culture, regionalism, and vernacular. Further, BoW methods fail on short text samples such as headlines or social media posts.
        - These shortcomings are potentially addressed by using word vectors that consider the context in which words are used, as shown by rheault and cochrane. Yet this relies on a sufficiently large volume of data to train an embedding model for each individual. This is a sufficiently large bar to clear that it is limited to political elites or particularly vocal members of the public that are likely not representative of the general population.
            - Not easy to implement
        - Surveys are expensive
        - sentiment analysis is not appropriate.
    - The fundamental challenge with these approaches is that they attempt to deconstruct language and create a model of the author's particular language use. While A few short sentences can communicate a great deal about someone's beliefs to a human, it is not enough data to create a representative model of the author's language. Humans succeed where current methods fail because humans are able to engage directly with the semantics of a text.
    - This paper overcomes this challenge by using large language models to classify documents based on their semantics and using a bayesian estimate of a count latent regression model to estimate ideal points. The result is an approach to ideological scaling that is broadly applicable across mediums and populations, and able to scale across specific dimensions defined by the researcher.

    - LLMs have in large part obviated the need to deconstruct language into bags of words or attempt to holistically model the language of particular groups or individuals by training custom word2vec or embedding models. 

Why semantic scaling?
    - short text with low samples. e.g. social media like Twitter, chat rooms, reddit, etc. short answer surveys.
    - tweetscores scales information consumption rather than ideology directly.
    - good methods of scaling from text in such a context are limited.
    - something that scales directly on revealed preferences.
    - separate ideological and affective dimensions.
    - explicit about what we are scaling on.
    - platform and population agnostic because text is generated across many mediums and populations.
    - Potential shortcoming is that it relies on revealed preferences

Approach
    - Short answer surveys as a touch point for conceptualizing the process. This twist is that individuals can answer questions as many times as they want within a given time period.
    - Model
        - Assumption is that users are more likely to make statements that entail premises they agree with than premises they do not agree with. To give an example, individuals that support Republicans are more likely to state that they support Republicans than to state that they do not support republicans. This assumption should be largely self evident and is largely parallel to the assumptions made in ideal point models that use voting or court opinions.
        - To express the idea more formally, suppose person i makes n statements about topic k. I assume that the number of statements that express conservative views about k is a function of person i's latent ideology theta.
        - Conventional scaling methods such as 2PL or factor analysis could be used by converting counts to majority class binary values or a ratio between conservative statements and all statements. However, this represents a significant loss of information.
        - Rather, I employ a two-parameter Conway Maxwell Poisson model expressed in slope intercept form as: formula. This model assumes the expected number of counts $\mu$ given by person i in response to item j is a function of the intercept b, item discrimination parameter alpha, and the latent "ability" parameter $\theta$.  In this instance, ability is an individuals propensity to make conservative statements.
            - Count IRT model specification. slope intercept form commonly used in mirt
        - However, an individuals propensity to make conservative statements is a function of not just their ideology, but also their propensity to make statements generally. To isolate the effect of these two parameters I use a CLRM model which estimates theta as a function of the intercept $\theta*$ and a vector of covariates. After accounting for other covariates that may impact ability to make conservative statements, $\theta*$ represents the individuals ideology. Here I add a single covariate, the average number of statements per item. This captures the individual's general propensity to make political statements. Thus, propensity to make conservative statements is a linear function of an individual's ideology and their general propensity to make statements.
        - Substituting this equation into the 2pcm we get: equation
        - Estimation with EM algorithm difficult due to dispersion and stability of estimates.
        - Bayesian estimate instead.
    - Identification and estimation
        - To identify the model I impose a standard normal prior on $\theta$. This ensures the model will produce a group of estimates centered near zero with a variance close to one. I then impose weakly informed priors in the form of C(0,5) to allow the algorithm broad range in exploring the posterior. 
        - The problem of reflection invariance still persists, meaning theta can be scaled by a factor of -1 without changing the model's prediction. This implies that higher levels of conservatism could be represented by either negative or positive values.
        - \citet{jackman2001multidimensional} demonstrates this problem can be resolved in the unidimensional scaling context by using starting values for theta in the expected direction of the scale. I thus use weakly informed prior values for theta. Individuals whose statements are classified as conservative more than half of the time are given a starting value of +1 and those whose statements are conservative less than half of the time are given a starting value of -1.
    - Entailment classification
        - To label documents I use the stance detection framework and methods outlined in Burnham 2023. Identifying the stance expressed in a document is an entailment classification task. formally defined, text sample T entails hypothesis H when a human reading T would infer that H is most likely true. This produces a binary classification indicating if the text does or does not entail the hypothesis. In the stance detection context, for example, we might have the following text sample and hypothesis pair:
            T: The Trump administration is delivering wins to the American people!
            H: The author of this text supports the Trump administration.
        From this example we would conclude the T entails H. 
        - One advantage of this approach is that it enables researchers to label documents at a large scale with relatively small investment. This is because many large language models have been pre-trained for entailment classification in a zero-shot (no training examples) and few-shot (few training examples) context. For example, rather than training a model for specifically identifying pro-Trump documents, we can pair documents about Trump with pro-Trump hypotheses and an entailment classifier will determine if the document entails the pro-Trump statement.
        - Some manually labeled documents are recommended to validate the results of the model, but the required labeling is orders of magnitude fewer than what training a model would require. It is also computationally more efficient because the models are pre-trained and a single entailment classifier can word for an arbitrary many dimensions.
        - Using this approach, a document labeling pipeline might consist of the following steps:
            1. Identify the items or topics along which a researcher wishes to scale.
            2. Categorize documents according to which item they are related to, perhaps by key words for short documents or a topic model for longer documents.
            3. Generate a set of hypothesis for each topic that encapsulate the stances that will be classified.
            4. Match documents to appropriate hypotheses and classify for entailment.
        - For example, one item I might wish to scale along is attitudes towards certain political identities or groups. I might then classify documents containing any of the words "conservative", "republican", or "GOP" as related to attitudes towards conservatives. To label documents as anti-conservative I can create tree variations of the same hypothesis:
            - The author of this text is against conservatives
            - The author of this text is against republicans
            - The author of this text is against the GOP
        And then match hypotheses to documents depending on which key word they contain. Documents that entail one of the hypotheses would be labeled as anti-conservative.
    
Data
    - Twitter
    - Reddit/youtube?
    - Congressional press releases?

Application: Affective vs. ideological polarization
    - Scholars distinguish between affective and ideological polarization. Definition. Research has shown that these are largely independent dimensions. 
    - This poses a challenge for many scaling approaches. Scholars may want to measure the dimensions independently and combining them may create measurement error. Further, it's not clear which dimension other scaling approaches are primarily capturing. 
    - Hypothesis: Affect based scaling will produce more distinct modes than ideologically based (Cite: Mason)

Results
- plots: density
- correlation with tweetscores
- people that post more may have stronger ideological preferences
- platform culture not to post certain beliefs


Congressional newsletters:
- Estimating congressional ideology offers several advantages:
    1. second point of validation via nominate scores
    2. Demonstration of application outside of Twitter.
    3. potentially interesting variance in results as MCs may deliberately depart from their voting record in their public statements due to either the cost associated with position taking or attempts to differentiate themselves to their constituents by aligning with certain factions within a party. Can show how affect is or is not correlated with policy preferences.
- Data collected:
    - Newsletters from the 117th congress. 
    - Affective dimensions remain the same.
    - Policy dimensions based on topic model of newsletters
    - Congress members that had at least 5 newsletters related to affect and 5 related to policy.
    - labeled documents containing key words related to the dimensions.

Nominate notes:
- argue that sincere voting takes place over strategic, however
- Also note it is consistent with cox and mccubbins model of agenda control.

Senate moderates and house extremists:
- pivotal politics model suggests moderates will have a lot of agenda setting power in small majority congresses. Nominate should be good at estimating their ideology
    -Senate: sinema, romney, murkowski, manchin, collins, shelley capito
    -House: cortez, omar, pressley, tlaib, bush
-Nomiante should be bad at the squad though

To do:
- scale based on policy endorsements
- show distribution of ideology on certain votes.
    
